Using Graph-Theoretic Machine Learning to Predict Human Driver Behavior

Studies have shown that autonomous vehicles (AVs) behave conservatively in a traffic environment composed of human drivers and do not adapt to local conditions and socio-cultural norms. It is known that socially aware AVs can be designed if there exists a mechanism to understand the behaviors of human drivers. We present an approach that leverages machine learning to predict, the behaviors of human drivers. This is similar to how humans implicitly interpret the behaviors of drivers on the road, by only observing the trajectories of their vehicles. We use graph-theoretic tools to extract driver behavior features from the trajectories and machine learning to obtain a computational mapping between the extracted trajectory of a vehicle in traffic and the driver behaviors. Compared to prior approaches in this domain, we prove that our method is robust, general, and extendable to broad-ranging applications such as autonomous navigation. We evaluate our approach on real-world traffic datasets captured in the U.S., India, China, and Singapore, as well as in simulation.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Sections/4-centrality.tex <==
\section{Centrality Measures}
\label{sec: centrality}
% \subsection{Use of Centrality Measures - What are Centrality Measures?}
% \input{Tables/centrality_cmetric}

 In graph theory and network analysis, centrality measures~\cite{rodrigues2019network} are real-valued functions $\zeta:\mathcal{V}\longrightarrow \mathbb{R}$, where $\mathcal{V}$ denotes the set of vertices and $\mathbb{R}$ denotes a scalar real number that identifies key vertices within a graph network. So far, centrality functions have been restricted to identifying influential personalities in online social media networks~\cite{cen-socialmedia} and key infrastructure nodes in the Internet~\cite{cen-internet}, to rank web-pages in search engines~\cite{cen-pagerank}, and to discover the origin of epidemics~\cite{cen-epidemic}. In this work, we show that centrality functions can measure the likelihood and intensity of different driver styles such as overspeeding, overtaking, sudden lane-changes, and weaving.
%  (See Table~\ref{tab: centrality_relationship}). 
 
There are several types of centrality functions. The ones that are of particular importance to us are the degree centrality and the closeness centrality. These centrality measures are defined in~\cite{cmetric} (See section III-C). Each function measures a different property of a vertex. Typically, the choice of selecting a centrality function depends on the current application at hand. For instance, in the examples mentioned earlier, the eigenvector centrality is used in search engines while the degree centrality is appropriate for measuring the popularity of an individual in social networks. Likewise, the centrality and the degree different centrality functions measure the likelihood and intensity of specific driving styles such as overspeeding, overtaking, sudden lane-changes, and weaving~\cite{cmetric}. 
% Here, we give the basic definitions of the key centrality functions used in our approach.

% \subsection{Relationship between Centrality and Driving Behavior}

% \input{Tables/centrality.tex}

% \begin{definition}
% \textbf{Closeness Centrality:} In a connected traffic-graph at time $t$ with adjacency matrix $A_t$, let $\mc{D}_t(v_i,v_j)$ denote the minimum total edge cost to travel from vertex $i$ to vertex $j$, then the discrete closeness centrality measure for the $i^\textrm{th}$ vehicle at time $t$ is defined as,
% \begin{equation}
%     \zeta^i_c[t] = \frac{N-1}{\sum_{v_j\in \mathcal{V}(t)\setminus \{v_i\}} \mc{D}_t(v_i,v_j)},
%     \label{eq: closeness}
% \end{equation}
% % where $v \in \mathcal{V}$ denote all vertices in the connected traffic-graph other than $u$.
% \end{definition}

% The closeness centrality for a given vertex computes the reciprocal of the sum of the edge values of the shortest paths between the given vertex and all other vertices in the connected traffic-graph. By definition, the higher the closeness centrality value, the more centrally the vertex is located in the graph. 
% % This idea is used to identify overtaking, sudden lane-changes, and weaving. If a vehicle, represented as a vertex in a traffic-graph, executes any of these styles, then the closeness centrality would oscillate between low values on the side lanes and high values towards the center. These styles, therefore, can be modeled by identifying the points of local minima (or maxima) of the centrality values. The same holds true for a conservative vehicle that would not tend to weave or zigzag through traffic. The closeness centrality values would remain approximately constant for conservative vehicles. We visualize the closeness centrality in Figure~\ref{fig: closeness_demo}.




% \begin{definition}
% \textbf{Degree Centrality:} In a connected traffic-graph at time $t$ with adjacency matrix $A_t$, let $\mc{N}_i(t) = \{ v_j \in \mc{V}(t), \ A_t(i,j) \neq 0, \nu_j \leq \nu_i\}$ denote the set of vehicles in the neighborhood of the $i^\textrm{th}$ vehicle with radius $\mu$, then the discrete degree centrality function of the $i^\textrm{th}$ vehicle at time $t$ is defined as,
% \begin{equation}
%     % \zeta_d(u) = \vts{ \{ A(u,v)\in A_{u,:} \land  \nu_u \geq \nu_v \} },
%     \begin{aligned}
%     \zeta^i_d[t] = \bigl | \{ v_j \in \mc{N}_i(t) \} \bigr | + \zeta^i_d[t-1] &\\
%     \textrm{such that} \ (v_i,v_j) \not\in \mc{E(\tau)}, \tau = 0, \ldots, t-1&
%     \end{aligned}
%     % \zeta_d(u) = 
%     \label{eq: degree}
% \end{equation}
% where $\vts{\cdot}$ denotes the cardinality of a set and $\nu_i, \nu_j$ denote the velocities of the $i^\textrm{th}$ and $j^\textrm{th}$ vehicles, respectively.
% \end{definition}

% The degree centrality at any time-step $t$ computes the cumulative number of edges between the given vertex and connected vertices in the traffic-graph over the past $t$ seconds, given that the velocity of the given vertex is higher than that of the connected vertices. 
% As $A_t$ is formed by adding rows and columns to $A_{t-1}$ (See equation~\ref{eq: A_update}), the degree of the $i^\textrm{th}$ vehicle (denoted as $\theta_i$) is calculated by simply counting the number of non-zero entries in the $i^\textrm{th}$ row of $A_t$. Let the rate of increase of $\theta_i$ be denoted as $\theta_i^{'}$. By definition of the degree centrality and construction of $A_t$, respectively, the degree centrality for an aggressively overspeeding vehicle will monotonically increase. Conversely, the degree centrality for a conservative vehicle driving at a uniform speed or braking often at unconventional spots such as green light intersections will be relatively flat. Figure~\ref{fig: degree_demo} visualizes how the degree centrality can distinguish between an overspeeding vehicle and a vehicle driving at a uniform speed. 

% \input{algorithm/algo1}


% \begin{definition}
% \textbf{Eigenvector Centrality:} In a connected traffic-graph at time $t$ with adjacency matrix $A_t$, the eigenvector centrality function is defined as,
% \begin{equation}
%     \zeta^i_e[t] = \frac{1}{\lambda} \sum_{v_j \in \mc{N}_i(t)}A_t(v_i,v_j)  \zeta^j_e[t] 
%     \label{eq: eigen}
% \end{equation}
% \end{definition}

% \noindent Here, $\lambda$ is the $k^{\textrm{th}}$ eigenvalue, and its corresponding eigenvector is denoted by $u_k$. Further, $\zeta^i_e$ represents the $i^{\textrm{th}}$ element of $u_k$. Therefore, vectorizing $\zeta^i_e$ for $i = 0, \ldots, N$ produces $u_k$ and it follows that $\zeta^i_e = u_k(i)$, where $u_k(i)$ denotes the $i^\textrm{th}$ element of $u_k$. 

% The eigenvectors of the laplacian matrix of the traffic-graph $\mc{G}_t$ measure the topology of the vertices in $\mc{G}_t$. The topology of vertex $v_i$ in a graph refers to the arrangement of its adjacent neighborhood $\mc{N}_i$. An example of a network topology is the star topology~\cite{star} with $v_i$ at the center if $(v_i, v_j) \in \mc{E}$ $\forall v_j \in \mc{N}_i$ and $(v_j, v_k) \notin \mc{E}$ $\forall \{v_j, v_k\} \in \mc{N}_i$. If we apply Definition~\ref{eq: eigen} to compute $u_k$, then we can additionally compute $w_k = Lu_k \in \mathbb{R}^{N}$ in which the $i^{\textrm{th}}$ entry (corresponding to the $i^\textrm{th}$ vehicle) of $w_k$ is given by,

% \begin{equation}
% \begin{split}
% w_k(i) &= D(i,i)u_k(i) - \sum_{v_j \in \mc{N}_i(t)} u_k(j)\\
% &= \sum_{v_j \in \mc{N}_i(t)} \brr{u_k(i)-u_k(j)}.    
% \end{split}
% \label{eq: topology}
% \end{equation}


% \noindent $w_k$ represents the sum of edge costs between the $i^\textrm{th}$ vehicle and all vehicles $v_j$ in the neighborhood of $v_i$. 

% Using Equation~\ref{eq: topology} and Equation~\ref{eq: eigen}, we can show the following,


% \begin{theorem}[Informal Theorem]
% Let $v_i$ and $v_j$ denote an aggressive and conservative vehicle, respectively. Then $w_k(i) \geq w_k(j)$.
% \end{theorem}

% We prove this result in the supplementary material.

% that aggressive vehicles produce a graph topology with larger edge lengths (Figure~\ref{fig: main} \textit{(right)}) while conservative vehicles tend to adhere to a uniform speed, thereby producing smaller edges of approximately uniform length (Figure~\ref{fig: main} \textit{(left)}). We prove this result in the Supplementary material.

% Thus, the $j^{\textrm{th}}$ entry of $w_i$ equals the sum of edge values of all edges with $v_j$ as the common node. Since the arrangement of vertices depend on the edge lengths between them, this determines the topology of the graph. In the GraphRQI model, $i=2$ is chosen to select the dominant eigenvector $u_2$ corresponding to the second-smallest eigenvalue to enforce smoothness in the resulting graphs. $u_2$ for each frame is computed and treated as a feature vector to train a multi-layer perceptron for behavior classification.

% \subsection{Relationship between Centrality and Driving Behavior}






==> Tables/list_of_behaviors.tex <==
\begin{table}%[tbhp]
\centering
\caption{A list showing the taxonomy of various aggressive and conservative behaviors. In this work, we focus on modeling the longitudinal and lateral specific styles (except ``tailgating'' and ``responding to pressure''). NA denotes ``Not Applicable''}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
Global Behavior & Specific Style/Indicator & Nature   \\
\midrule
\multirow{7}{*}{Aggressive} & Overspeeding  & Longitudinal\\
&  Tailgating & Longitudinal\\
& Overtake as much as possible & Lateral\\
 & Weaving & Lateral \\
& Sudden Lane-Changes & Lateral\\
& Inappropriate use of horn & NA\\
 &  Flashing lights at vehicle in front & NA\\
\midrule
\multirow{3}{*}{Conservative} & Uniform speed or under-speeding & Longitudinal \\
 & Conforms to single lane & Lateral \\
 & Responding to pressure from other drivers & NA \\

% Laplacian Centrality &  Degree of ``agitation'' &  High (Agg.) or Low (Con.)\\
\bottomrule
\end{tabular}
}
\label{tab: list_of_behaviors}
% \vspace{-10pt}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\end{table}

==> algorithm/algo1.tex <==
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetKwComment{Comment}{$\triangleright$\ }{}
\SetAlgoLined
\Input{$u = v_i \gets [x_i,y_i]^\top \ \forall v_i \in \mathcal{V}(t)$}
\Output{$\textrm{SLE}(t), \textrm{SIE}(t)$}
$t=0$\\
\For {each $v \in \mathcal{V}(t)$}{
\While{$t \leq T$}{ 
// Compute Centrality //\\
$     \zeta^i_c[t] = \frac{N-1}{\Tstrutfrac \sum_{v_j\in \mathcal{V}(t)\setminus \{v_i\}} \mc{D}_t(v_i,v_j)}$ \\ 
$    \zeta^i_d[t] = \bigl | \{ v_j \in \mc{N}_i(t) \} \bigr | + \zeta^i_d[t-1], (v_i,v_j) \not\in \mc{E(\tau)}, \tau = 0, \ldots, t-1$ \\
% $         \zeta^i_e[t] = \frac{1}{\lambda} \sum_{v_j \in \mc{\mc{N}_i}(t)}A_t(v_i,v_j)  \zeta^j_e[t] $\\
$t \gets t+1$ \\
// Perform Polynomial Regression w.r.t Time //\\
$\beta = \argmin_\beta \Vts{\zeta - M\beta}$\\
$\zeta(t) = \beta_0 + \beta_1 t + \beta_2t^2$\\
// Compute Likelihood and Intensity //\\
% Form $\cm$ using Definition~\ref{def: cmetric}\\
\For{$k=0,1,2$}{
$\textrm{SLE}_k(t) = \abs*{\frac{\partial \zeta(t)}{\partial t}}$\\
$\textrm{SIE}_k(t) = \abs*{\frac{\partial^2 \zeta(t)}{\partial t^2}}$
}
}
}
\caption{Our approach outputs the Style Likelihood Estimate (SLE) and Style Intensity Estimate (SIE) for a vehicle, $u$, in a given time-period $\Delta t$. }
\label{alg: main}
% \vspace{-5pt}
\end{algorithm}



==> img/inverse_curves.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[h]{.49\linewidth}
  \includegraphics[width=\linewidth]{img/UScurve.jpg}
\caption{Lateral styles (higher TDE) versus longitudinal styles (lower TDE)}
\label{fig: UScurve}
\end{subfigure}
%
\begin{subfigure}[h]{.49\linewidth}
  \includegraphics[width=\linewidth]{img/SGcurve.jpg}
\caption{Lateral styles (higher TDE) versus longitudinal styles (lower TDE)}
\label{fig: SGcurve}
\end{subfigure}
%
\begin{subfigure}[h]{.49\linewidth}
  \includegraphics[width=\linewidth]{img/BJcurve.jpg}
\caption{Longitudinal styles (higher TDE) versus lateral styles (lower TDE)}
\label{fig: CHcurve}
\end{subfigure}
%
\begin{subfigure}[h]{.49\linewidth}
  \includegraphics[width=\linewidth]{img/INDcurve.jpg}
\caption{Longitudinal styles (higher TDE) versus lateral styles (lower TDE)}
\label{fig: INDcurve}
\end{subfigure}
% \centering
\caption{\textbf{Inverse Relationship:} We observe an inverse correlation between the TDE and the type of style (longitudinal vs. lateral). The ``type of style'' on the x-axis is a continuous variable. For example, a vehicle may simultaneously overspeed \textit{and} perform a lane-change. The ``type'' of this style would lie somewhere along the middle of the x-axis. (\textit{Top row}) The U.S. and Singapore are countries with low traffic density and lack of heterogeneity, and so drivers are more likely to perform longitudinal driving styles (Section~\ref{sec: culture_analysis}). Therefore StylePredict can model longitudinal styles more accurately (lower TDE) than lateral styles (higher TDE). (\textit{Bottom row}) Conversely, India and China are countries with higher traffic density and heterogeneity, and so drivers are less likely to perform longitudinal driving styles and more likely to perform lateral styles (Section~\ref{sec: culture_analysis}). Therefore, StylePredict can model lateral styles more accurately (lower TDE) than longitudinal styles (higher TDE).  } 
\label{fig: inverse_curve}
% \vspace{-10pt}
\end{figure*}
